ByteNet: Rethinking Multimedia File Fragment Classification through Visual Perspectives

Multimedia file fragment classification (MFFC) aims to identify file fragment types, e.g., image/video, audio, and text without system metadata. It is of vital importance in multimedia storage and communication. Existing MFFC methods typically treat fragments as 1D byte sequences and emphasize the relations between separate bytes (interbytes) for classification. However, the more informative relations inside bytes (intrabytes) are overlooked and seldom investigated. By looking inside bytes, the bit-level details of file fragments can be accessed, enabling a more accurate classification. Motivated by this, we first propose Byte2Image, a novel visual representation model that incorporates previously overlooked intrabyte information into file fragments and reinterprets these fragments as 2D grayscale images. This model involves a sliding byte window to reveal the intrabyte information and a rowwise stacking of intrabyte ngrams for embedding fragments into a 2D space. Thus, complex interbyte and intrabyte correlations can be mined simultaneously using powerful vision networks. Additionally, we propose an end-to-end dual-branch network ByteNet to enhance robust correlation mining and feature representation. ByteNet makes full use of the raw 1D byte sequence and the converted 2D image through a shallow byte branch feature extraction (BBFE) and a deep image branch feature extraction (IBFE) network. In particular, the BBFE, composed of a single fully-connected layer, adaptively recognizes the co-occurrence of several some specific bytes within the raw byte sequence, while the IBFE, built on a vision Transformer, effectively mines the complex interbyte and intrabyte correlations from the converted image. Experiments on the two representative benchmarks, including 14 cases, validate that our proposed method outperforms state-of-the-art approaches on different cases by up to 12.2%.

==> data/Breakdown.tex <==
\begin{tabular}{llcccccccccc} 
% \begin{tabular}{lllllll} 
\hline
\multirow{2}{*}{Filetype}  & \multirow{2}{*}{Tag}  &  \multicolumn{5}{c}{SS=512} & \multicolumn{5}{c}{SS=4,096} \\ \cmidrule{3-12}
&  &  NN-CO & FiFTy & CNN+LTSM & ByteResNet & ByteFormer &  NN-CO & FiFTy & CNN+LTSM & ByteResNet & ByteFormer   \\ \hline  

% ARW & Raw &  97.8 & 97.8 & 96.4 & & &   98.8 & 98.9 & 98.3 \\ 
% CR2 & Raw &   82.4 & 86.7 & 87.6 & & &   95.3 & 96.1 & 97.0 \\ 
% DNG & Raw &   81.6 & 82.7 & 80.0 & & &   96.7 & 96.1 & 97.0\\ 
% GPR & Raw &    98.7 & 99.2 & 99.4 & & &  99.5 & 99.9 & 99.9 \\
% NEF & Raw &   89.3 & 87.7 & 86.4  & & &   89.0 & 95.3 & 95.6 \\
% NRW & Raw &   96.1 & 96.9 & 95.0 & & &   96.7 & 97.7 & 98.0 \\
% ORF & Raw &   84.0 & 86.3 & 87.4 & & &   97.6 & 96.3 & 96.9 \\
% PEF & Raw &   96.1  & 95.1 & 94.3 & & &    98.9 & 99.1 & 99.2 \\
% RAF & Raw &    97.9 & 98.3 & 98.6 & & &   91.3 & 87.1 & 89.4 \\
% RW2 & Raw &    96.6 & 96.5 & 93.8 & & & 97.9 & 97.9 & 98.0 \\
% 3FR & Raw &  99.4 & 99.6 & 99.8 & & &    92.6 & 99.5 & 99.6 \\

% JPG & Bitmap & 53.2 & 83.5 & 87.0 & & & 48.6 & 86.3 & 90.3 \\
% TIFF & Bitmap & 90.0 & 96.1 & 95.6 & & & 98.6 & 99.0 & 97.4 \\
% HEIC & Bitmap & 2.0 & 31.7  & 36.2 & & & 4.0 & 49.5 & 46.5 \\
% BMP & Bitmap & 97.5 & 98.0 & 98.1 & & & 99.4 & 98.4 & 99.6 \\
% GIF & Bitmap & 84.5 & 93.5 & 93.6 & & & 98.5 & 99.1 & 99.3 \\
% PNG & Bitmap & 47.6 & 67.2 & 74.2 & & & 72.9 & 88.0 & 85.4 \\

% AI & Vector & 25.5 & 23.3 & 25.0 &&& 50.9 & 57.7 & 55.4 \\
% EPS & Vector & 98.8 & 98.7 & 98.8 &&& 98.0 & 95.8 & 99.0 \\
% PSD & Vector & 93.7 & 95.3 & 95.4 &&& 95.6 & 95.9 & 96.0 \\

ARW & Raw & 97.8 & 97.8 & 96.4 & & & 98.8 & 98.9 & 98.3 & & \\
CR2 & Raw & 82.4 & 86.7 & 87.6 & & & 95.3 & 94.8 & 95.6 & & \\
DNG & Raw & 81.6 & 82.7 & 80.0 & & & 96.7 & 96.1 & 97.0 & & \\
GPR & Raw & 98.7 & 99.2 & 99.4 & & & 99.5 & 99.9 & 99.9 & & \\
NEF & Raw & 89.3 & 87.7 & 86.4 & & & 89.0 & 95.3 & 95.6 & & \\
NRW & Raw & 96.1 & 96.9 & 95.0 & & & 96.7 & 97.7 & 98.0 & & \\
ORF & Raw & 84.0 & 86.3 & 87.4 & & & 97.6 & 96.3 & 96.9 & & \\
PEF & Raw & 96.1 & 95.1 & 94.3 & & & 98.9 & 99.1 & 99.2 & & \\
RAF & Raw & 97.9 & 98.3 & 98.6 & & & 91.3 & 87.1 & 89.4 & & \\
RW2 & Raw & 96.6 & 96.5 & 93.8 & & & 97.9 & 97.9 & 98.0 & & \\
3FR & Raw & 99.4 & 99.6 & 99.8 & & & 92.6 & 99.5 & 99.6 & & \\

JPG & Bitmap & 77.5 & 83.5 & 87.0 & & & 92.5 & 86.3 & 90.3 & & \\
TIFF & Bitmap & 90.0 & 96.1 & 95.6 & & & 98.6 & 99.0 & 97.4 & & \\
HEIC & Bitmap & 2.0 & 31.7 & 36.2 & & & 4.0 & 49.5 & 46.5 & & \\
BMP & Bitmap & 97.5 & 98.0 & 98.1 & & & 99.4 & 98.4 & 99.6 & & \\
GIF & Bitmap & 84.5 & 93.5 & 93.6 & & & 98.5 & 99.1 & 99.3 & & \\
PNG & Bitmap & 47.6 & 67.2 & 74.2 & & & 72.9 & 88.0 & 85.4 & & \\

AI & Vector & 25.5 & 23.3 & 25.0 & & & 50.9 & 57.7 & 55.4 & & \\
EPS & Vector & 98.8 & 98.7 & 98.8 & & & 98.0 & 95.8 & 99.0 & & \\
PSD & Vector & 93.7 & 95.3 & 95.4 & & & 95.6 & 95.9 & 96.0 & & \\

MOV & Video & 8.7 & 6.1 & 15.2 & & & 0.0 & 18.5 & 16.5 & & \\
MP4 & Video & 14.8 & 1.6 & 12.3 & & & 62.2 & 71.8 & 68.5 & & \\
3GP & Video & 91.6 & 85.6 & 86.0 & & & 98.8 & 98.1 & 98.9 & & \\
AVI & Video & 13.8 & 10.9 & 14.8 & & & 64.9 & 67.1 & 70.1 & & \\
MKV & Video & 90.5 & 88.0 & 88.0 & & & 99.1 & 98.4 & 99.3 & & \\
OGV & Video & 67.4 & 57.3 & 65.0 & & & 94.5 & 94.9 & 94.9 & & \\
WEBM & Video & 39.6 & 39.8 & 42.7 & & & 71.5 & 78.1 & 79.5 & & \\

APK & Archive & 32.5 & 29.9 & 31.2 & & & 48.3 & 49.7 & 47.4 & & \\
JAR & Archive & 36.3 & 41.2 & 44.3 & & & 74.8 & 73.8 & 74.0 & & \\
MSI & Archive & 5.1 & 10.1 & 9.8 & & & 26.6 & 60.1 & 57.5 & & \\
DMG & Archive & 7.0 & 18.2 & 16.4 & & & 17.4 & 19.4 & 24.8 & & \\
7Z & Archive & 0.9 & 0.0 & 7.6 & & & 53.2 & 0.1 & 23.2 & & \\
BZ2 & Archive & 8.6 & 13.9 & 11.6 & & & 75.8 & 80.6 & 82.6 & & \\
DEB & Archive & 9.9 & 13.8 & 12.7 & & & 1.5 & 0.8 & 2.9 & & \\
GZ & Archive & 11.3 & 13.2 & 15.0 & & & 53.0 & 42.1 & 55.1 & & \\
PKG & Archive & 5.6 & 4.5 & 7.3 & & & 41.0 & 62.7 & 57.5 & & \\
RAR & Archive & 13.0 & 24.0 & 23.6 & & & 18.0 & 46.6 & 39.4 & & \\
RPM & Archive & 7.9 & 13.6 & 12.5 & & & 10.7 & 21.9 & 22.4 & & \\
XZ & Archive & 0.0 & 0.0 & 6.1 & & & 0.0 & 12.1 & 9.5 & & \\
ZIP & Archive & 16.2 & 13.8 & 15.1 & & & 36.6 & 34.2 & 38.5 & & \\

EXE & Executable & 9.2 & 0.3 & 6.8 & & & 4.3 & 2.7 & 4.9 & & \\
MACH-O & Executable & 93.6 & 92.6 & 94.2 & & & 95.7 & 95.0 & 96.0 & & \\
ELF & Executable & 87.6 & 85.9 & 87.6 & & & 92.2 & 86.4 & 92.8 & & \\
DLL & Executable & 91.7 & 91.1 & 92.2 & & & 94.4 & 91.7 & 94.5 & & \\

DOC & Office & 91.4 & 87.2 & 89.0 & & & 91.6 & 88.9 & 90.0 & & \\
DOCX & Office & 14.7 & 19.4 & 17.7 & & & 49.9 & 60.6 & 63.4 & & \\
KEY & Office & 35.8 & 44.1 & 44.3 & & & 56.7 & 43.1 & 49.8 & & \\
PPT & Office & 44.2 & 41.3 & 38.2 & & & 58.4 & 53.5 & 55.6 & & \\
PPTX & Office & 38.3 & 44.4 & 41.3 & & & 32.7 & 36.0 & 37.5 & & \\
XLS & Office & 99.4 & 99.3 & 99.5 & & & 99.2 & 99.3 & 99.5 & & \\
XLSX & Office & 96.8 & 95.2 & 96.9 & & & 97.4 & 97.2 & 98.0 & & \\

DJVU & Published & 18.0 & 24.6 & 22.8 & & & 34.8 & 30.4 & 40.8 & & \\
EPUB & Published & 29.3 & 20.7 & 24.8 & & & 74.3 & 79.7 & 80.0 & & \\
MOBI & Published & 72.5 & 72.4 & 73.0 & & & 74.4 & 73.7 & 74.7 & & \\
PDF & Published & 21.9 & 23.1 & 22.2 & & & 48.3 & 45.8 & 46.7 & & \\

MD & Human-readable & 98.0 & 97.1 & 97.4 & & & 99.9 & 97.4 & 99.9 & & \\
RTF & Human-readable & 99.5 & 99.7 & 99.7 & & & 100.0 & 99.8 & 100.0 & & \\
TXT & Human-readable & 95.0 & 93.7 & 93.4 & & & 92.9 & 93.0 & 93.2 & & \\
TEX & Human-readable & 97.8 & 97.6 & 97.9 & & & 98.8 & 98.3 & 98.9 & & \\
JSON & Human-readable & 99.8 & 99.5 & 99.6 & & & 100.0 & 99.8 & 99.9 & & \\
HTML & Human-readable & 98.4 & 97.5 & 97.6 & & & 99.5 & 99.6 & 99.5 & & \\
XML & Human-readable & 100.0 & 100.0 & 100.0 & & & 100.0 & 100.0 & 100.0 & & \\
LOG & Human-readable & 100.0 & 99.9 & 100.0 & & & 99.9 & 99.9 & 99.9 & & \\
CSV & Human-readable & 99.9 & 99.6 & 99.6 & & & 99.0 & 99.7 & 99.6 & & \\

AIFF & Audio & 95.7 & 99.4 & 99.7 & & & 94.5 & 98.8 & 99.0 & & \\
FLAC & Audio & 66.9 & 74.2 & 70.4 & & & 87.8 & 97.9 & 95.6 & & \\
M4A & Audio & 92.6 & 94.3 & 97.3 & & & 96.5 & 98.2 & 98.3 & & \\
MP3 & Audio & 94.0 & 94.4 & 95.0 & & & 98.9 & 98.9 & 99.0 & & \\
OGG & Audio & 84.2 & 90.4 & 90.3 & & & 95.4 & 95.5 & 96.0 & & \\
WAV & Audio & 99.9 & 100.0 & 100.0 & & & 74.0 & 98.7 & 98.8 & & \\
WMA & Audio & 99.2 & 98.2 & 98.7 & & & 99.9 & 99.9 & 99.9 & & \\
PCAP & Misc & 55.4 & 51.0 & 49.3 & & & 95.6 & 95.4 & 95.5 & & \\
TIF & Misc & 98.1 & 98.1 & 98.7 & & & 99.2 & 99.3 & 99.4 & & \\
DWG & Misc & 96.5 & 96.2 & 96.3 & & & 98.8 & 96.9 & 98.8 & & \\
SQLITE & Misc & 98.9 & 98.6 & 99.4 & & & 99.5 & 99.8 & 98.5 & & \\
\multicolumn{2}{c}{Total Wins} & 25 & & \\ \hline

\end{tabular}

==> data/Generalization.tex <==
\begin{tabular}{llcccccc}
\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{6}{c}{ Accuracy (\%) in Scene } \\ 
\cline { 3 - 8 } & & $\# 1$ & $\# 2$ & $\# 3$ & $\# 4$ & $\# 5$ & $\# 6$  \\

\hline \multirow{4}{*}{\shortstack{DFRWS \\ SS=512}} & FiFTy & $\mathbf{41.4}$ & $\mathbf{46.5}$ & 60.8 & 71.9 & $\mathbf{86.8}$ & 78.1  \\
& DSCNN & 36.5 & 20.8 & 64.3 & 69.8 & 77.6 & 80.7  \\ 
\cdashline{2-8}
& ByteResNet & 63.0 & 76.5 & 77.9 & 84.5 &  &  74.2  \\
& ByteFormer & & &&&&  \\
\hline 

\multirow{4}{*}{\shortstack{GovDocs \\ SS=4096}} & FiFTy & 55.9 & 45.2 & 83.9 & 88.0 & 88.3 & 82.3 \\
& DSCNN & 63.0 & 76.5 & 77.9 & 84.5 & 90.9 & 97.3 \\   
\cdashline{2-8}
& ByteResNet & & &&&&  \\
& ByteFormer & & &&&&  \\
\hline
\end{tabular}

==> data/VFF.tex <==

\belowrulesep=0pt
\aboverulesep=0pt

\begin{tabular}{|l|cc|cc|} 
\hline
\multirow{2}{*}{Method}  &  \multicolumn{2}{c|}{SS = 512}  &\multicolumn{2}{c|}{SS = 4,096}\\ \cmidrule{2-5}
 & Acc. & JPEG Acc.   & Acc. & JPEG Acc.  \\ \hline  \hline
Byte2Vec+kNN~\cite{haque2022byte}& 61.1 & 52.2 & 67.3 & 57.3  \\
FiFTy~\cite{mittal2020fifty}  & 68.0 &  \textcolor{blue}{72.8} & 66.6 & \textcolor{red}{70.1}  \\ 
DSCNN~\cite{saaim2022light} & 74.5 & \textcolor{red}{80.4} &  \ 78.2 & 84.2 \\ \hdashline
ByteResNet (Ours) &  \textcolor{blue}{74.9}  & 67.4 &  \textcolor{blue}{78.5} & 64.6\\ 
ByteFormer (Ours) & \textcolor{red}{78.1}  &  70.9  &  79.2 &  \textcolor{blue}{72.8}  \\ \hline   
\end{tabular}



==> data/n-gram.tex <==

\begin{tabular}{|l|l|cccc|} 
\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{4}{c|}{Accuracy (\%) in $N$-gram } \\ \cline {3 - 6} 
 & & 2 & 4 & 8 & 16   \\ \hline \hline
\multirow{2}{*}{FFT-75} & ByteResNet & 90.4 & 90.5 & 90.3 & 90.4 \\  %90.5
 & ByteFormer & 89.8 & 90.4 & 90.8 & 91.1 \\  % scen2 FiFty 512  
 \hline   \hline
\multirow{2}{*}{VFF-16}  & ByteResNet  & 74.9 & 75.3  & 75.1 & 74.9 \\
 & ByteFormer & 74.2 & 74.8 & 75.7 & 78.1  \\ \hline

\end{tabular}
